The Age of Synthetic Realities: Challenges and Opportunities

Synthetic realities are digital creations or augmentations that are contextually generated through the use of Artificial Intelligence (AI) methods, leveraging extensive amounts of data to construct new narratives or realities, regardless of the intent to deceive. In this paper, we delve into the concept of synthetic realities and their implications for Digital Forensics and society at large within the rapidly advancing field of AI. We highlight the crucial need for the development of forensic techniques capable of identifying harmful synthetic creations and distinguishing them from reality. This is especially important in scenarios involving the creation and dissemination of fake news, disinformation, and misinformation. Our focus extends to various forms of media, such as images, videos, audio, and text, as we examine how synthetic realities are crafted and explore approaches to detecting these malicious creations. Additionally, we shed light on the key research challenges that lie ahead in this area. This study is of paramount importance due to the rapid progress of AI generative techniques and their impact on the fundamental principles of Forensic Science.

==> sections/next-ten.tex <==


\textcolor{red}{Sebastien: WiP}

% 1-page with your views as for how you think we could improve forensic and biometric systems in the future to protect ourselves --- in other words, research paths possible. 

Synthetic realities offer challenging problems and research directions across various disciplines such as 
signal processing, computer vision, natural language processing, machine learning, 
criminalistics (Forensic science),
linguistics, psychology and neuroscience. 
 
\begin{enumerate}
    \item \textbf{detection}:
    new methods need to be created to generalize to unseen attack vectors;
    \item \textbf{attribution}: 
    new open-set recognition paradigms need to be invented to discover unknown attack vectors; 
    \item \textbf{explainability}: 
    new technologies need to proposed to automatically describe cues or inconsistencies in natural language;
    new studies on the use of likelihood ratio (LR) to evaluate evidence in the context of synthetic realities need to be undertaken;
\end{enumerate}

%Topics of Interest from the call https://www.computer.org/digital-library/magazines/sp/synthetic-realities-ai-generated-contents
%- Detection of synthetic realities (text, image, videos, audio, etc.) by machines or humans
%- Challenges for Forensics and Security in the age of synthetic realities 
%- Possible policies and regulation that should or could be discussed regarding AI-generated or enabled content and synthetic realities 
%- What does the future look like in this new context of AI-generated contents? 
%- Synthetic realities and the metaverse
%- DeepFakes and their disruptions 
%- AI-generated Spoofing Attacks 
%- What’s next for AI-generated content and the creation of synthetic realities? 
%- New practices for Forensics and Security with the presence of Synthetic Realities 

